Fractional Perimeter and Nonlocal Minimal Surfaces

This Master's thesis presents a study of the basic properties of the s-fractional perimeter and of the regularity theory of the corresponding s-minimal sets. In particular, we give full detailed proofs for all the Theorems contained in the article "Nonlocal Minimal Surfaces" by Caffarelli, Roquejoffre and Savin, where these s-minimal sets were introduced and studied for the first time.

==> glyphtounicode-cmr.tex <==
%
% Copyright (c) 2008,  Han The Thanh <thanh@river-valley.org>
% Copyright (c) 2014,  Peter Selinger <selinger@mathstat.dal.ca>
%                      
%  This file may be distributed and/or modified under the conditions
%  of the LaTeX Project Public License, either version 1.2 of this
%  license or (at your option) any later version.  The latest version
%  of this license is in:
%    
%    http://www.latex-project.org/lppl.txt
%    
%  and version 1.2 or later is part of all distributions of LaTeX
%  version 1999/12/01 or later.
%
% Changes:
% 2014/08/11: PS1 - mapped most glyphs to existing Unicode code points.
% 2014/08/11: PS1 - added mappings for the xyatip and xybtip fonts.

%% Glyphs from the cmex fonts:

\pdfglyphtounicode{angbracketleftBig}{27E8}
\pdfglyphtounicode{angbracketleftBigg}{27E8}
\pdfglyphtounicode{angbracketleftbig}{27E8}
\pdfglyphtounicode{angbracketleftbigg}{27E8}
\pdfglyphtounicode{angbracketrightBig}{27E9}
\pdfglyphtounicode{angbracketrightBigg}{27E9}
\pdfglyphtounicode{angbracketrightbig}{27E9}
\pdfglyphtounicode{angbracketrightbigg}{27E9}
\pdfglyphtounicode{arrowbt}{2193}
\pdfglyphtounicode{arrowdblbt}{21D3}
\pdfglyphtounicode{arrowdbltp}{21D1}
\pdfglyphtounicode{arrowhookleft}{21AA}
\pdfglyphtounicode{arrowhookright}{21A9}
\pdfglyphtounicode{arrowtp}{2191}
\pdfglyphtounicode{arrowvertex}{23D0}
\pdfglyphtounicode{arrowvertexdbl}{ED12}
\pdfglyphtounicode{backslashBig}{005C}
\pdfglyphtounicode{backslashBigg}{005C}
\pdfglyphtounicode{backslashbig}{005C}
\pdfglyphtounicode{backslashbigg}{005C}
\pdfglyphtounicode{braceex}{23AA}
\pdfglyphtounicode{bracehtipdownleft}{ED17}
\pdfglyphtounicode{bracehtipdownright}{ED18}
\pdfglyphtounicode{bracehtipupleft}{ED19}
\pdfglyphtounicode{bracehtipupright}{ED1A}
\pdfglyphtounicode{braceleftBig}{007B}
\pdfglyphtounicode{braceleftBigg}{007B}
\pdfglyphtounicode{braceleftbig}{007B}
\pdfglyphtounicode{braceleftbigg}{007B}
\pdfglyphtounicode{braceleftbt}{23A9}
\pdfglyphtounicode{braceleftmid}{23A8}
\pdfglyphtounicode{bracelefttp}{23A7}
\pdfglyphtounicode{bracerightBig}{007D}
\pdfglyphtounicode{bracerightBigg}{007D}
\pdfglyphtounicode{bracerightbig}{007D}
\pdfglyphtounicode{bracerightbigg}{007D}
\pdfglyphtounicode{bracerightbt}{23AD}
\pdfglyphtounicode{bracerightmid}{23AC}
\pdfglyphtounicode{bracerighttp}{23AB}
\pdfglyphtounicode{bracketleftBig}{005B}
\pdfglyphtounicode{bracketleftBigg}{005B}
\pdfglyphtounicode{bracketleftbig}{005B}
\pdfglyphtounicode{bracketleftbigg}{005B}
\pdfglyphtounicode{bracketleftbt}{23A3}
\pdfglyphtounicode{bracketleftex}{23A2}
\pdfglyphtounicode{bracketlefttp}{23A1}
\pdfglyphtounicode{bracketrightBig}{005D}
\pdfglyphtounicode{bracketrightBigg}{005D}
\pdfglyphtounicode{bracketrightbig}{005D}
\pdfglyphtounicode{bracketrightbigg}{005D}
\pdfglyphtounicode{bracketrightbt}{23A6}
\pdfglyphtounicode{bracketrightex}{23A5}
\pdfglyphtounicode{bracketrighttp}{23A4}
\pdfglyphtounicode{ceilingleftBig}{2308}
\pdfglyphtounicode{ceilingleftBigg}{2308}
\pdfglyphtounicode{ceilingleftbig}{2308}
\pdfglyphtounicode{ceilingleftbigg}{2308}
\pdfglyphtounicode{ceilingrightBig}{2309}
\pdfglyphtounicode{ceilingrightBigg}{2309}
\pdfglyphtounicode{ceilingrightbig}{2309}
\pdfglyphtounicode{ceilingrightbigg}{2309}
\pdfglyphtounicode{circledotdisplay}{2A00}
\pdfglyphtounicode{circledottext}{2A00}
\pdfglyphtounicode{circlemultiplydisplay}{2A02}
\pdfglyphtounicode{circlemultiplytext}{2A02}
\pdfglyphtounicode{circleplusdisplay}{2A01}
\pdfglyphtounicode{circleplustext}{2A01}
\pdfglyphtounicode{contintegraldisplay}{222E}
\pdfglyphtounicode{contintegraltext}{222E}
\pdfglyphtounicode{coproductdisplay}{2210}
\pdfglyphtounicode{coproducttext}{2210}
\pdfglyphtounicode{floorleftBig}{230A}
\pdfglyphtounicode{floorleftBigg}{230A}
\pdfglyphtounicode{floorleftbig}{230A}
\pdfglyphtounicode{floorleftbigg}{230A}
\pdfglyphtounicode{floorrightBig}{230B}
\pdfglyphtounicode{floorrightBigg}{230B}
\pdfglyphtounicode{floorrightbig}{230B}
\pdfglyphtounicode{floorrightbigg}{230B}
\pdfglyphtounicode{hatwide}{02C6}
\pdfglyphtounicode{hatwider}{02C6}
\pdfglyphtounicode{hatwidest}{02C6}
\pdfglyphtounicode{integraldisplay}{222B}
\pdfglyphtounicode{integraltext}{222B}
\pdfglyphtounicode{intersectiondisplay}{22C2}
\pdfglyphtounicode{intersectiontext}{22C2}
\pdfglyphtounicode{logicalanddisplay}{22C0}
\pdfglyphtounicode{logicalandtext}{22C0}
\pdfglyphtounicode{logicalordisplay}{22C1}
\pdfglyphtounicode{logicalortext}{22C1}
\pdfglyphtounicode{mapsto}{21A6}
\pdfglyphtounicode{parenleftBig}{0028}
\pdfglyphtounicode{parenleftBigg}{0028}
\pdfglyphtounicode{parenleftbig}{0028}
\pdfglyphtounicode{parenleftbigg}{0028}
\pdfglyphtounicode{parenleftbt}{239D}
\pdfglyphtounicode{parenleftex}{239C}
\pdfglyphtounicode{parenlefttp}{239B}
\pdfglyphtounicode{parenrightBig}{0029}
\pdfglyphtounicode{parenrightBigg}{0029}
\pdfglyphtounicode{parenrightbig}{0029}
\pdfglyphtounicode{parenrightbigg}{0029}
\pdfglyphtounicode{parenrightbt}{23A0}
\pdfglyphtounicode{parenrightex}{239F}
\pdfglyphtounicode{parenrighttp}{239E}
\pdfglyphtounicode{productdisplay}{220F}
\pdfglyphtounicode{producttext}{220F}
\pdfglyphtounicode{radicalBig}{221A}
\pdfglyphtounicode{radicalBigg}{221A}
\pdfglyphtounicode{radicalbig}{221A}
\pdfglyphtounicode{radicalbigg}{221A}
\pdfglyphtounicode{radicalbt}{221A}
\pdfglyphtounicode{radicaltp}{ED6A}
\pdfglyphtounicode{radicalvertex}{ED6B}
\pdfglyphtounicode{slashBig}{002F}
\pdfglyphtounicode{slashBigg}{002F}
\pdfglyphtounicode{slashbig}{002F}
\pdfglyphtounicode{slashbigg}{002F}
\pdfglyphtounicode{summationdisplay}{2211}
\pdfglyphtounicode{summationtext}{2211}
\pdfglyphtounicode{tie}{2040}
\pdfglyphtounicode{tildewide}{02DC}
\pdfglyphtounicode{tildewider}{02DC}
\pdfglyphtounicode{tildewidest}{02DC}
\pdfglyphtounicode{uniondisplay}{22C3}
\pdfglyphtounicode{unionmultidisplay}{2A04}
\pdfglyphtounicode{unionmultitext}{2A04}
\pdfglyphtounicode{unionsqdisplay}{2A06}
\pdfglyphtounicode{unionsqtext}{2A06}
\pdfglyphtounicode{uniontext}{22C3}
\pdfglyphtounicode{vextenddouble}{ED79}
\pdfglyphtounicode{vextendsingle}{23D0}

%% Glyphs from the cmr fonts:

\pdfglyphtounicode{suppress}{EB61}

%% Glyphs from the lasy fonts:

%% Note: unfortunately, some other fonts, such as line and xydash,
%% also use glyphs names a0...a127, but for different glyphs.

\pdfglyphtounicode{a1}{25C1}
\pdfglyphtounicode{a2}{22B4}
\pdfglyphtounicode{a3}{25B7}
\pdfglyphtounicode{a4}{22B5}
\pdfglyphtounicode{a40}{02C2}
\pdfglyphtounicode{a41}{02C3}
\pdfglyphtounicode{a42}{2303}
\pdfglyphtounicode{a43}{2304}
\pdfglyphtounicode{a48}{2127}
\pdfglyphtounicode{a49}{22C8}
\pdfglyphtounicode{a50}{25A1}
\pdfglyphtounicode{a51}{25C7}
\pdfglyphtounicode{a58}{2053}
\pdfglyphtounicode{a59}{219D}
\pdfglyphtounicode{a60}{228F}
\pdfglyphtounicode{a61}{2290}

%% Glyphs from the xyatip and xybtip fonts fonts of the XYPic package.
%% They denote half arrow tips pointing in various directions.  We map
%% them to Unicode arrows pointing in approximately the same
%% direction, in increments of 45 degrees.

\pdfglyphtounicode{d0}{2199}
\pdfglyphtounicode{d1}{2199}
\pdfglyphtounicode{d2}{2199}
\pdfglyphtounicode{d3}{2199}
\pdfglyphtounicode{d4}{2199}
\pdfglyphtounicode{d5}{2199}
\pdfglyphtounicode{d6}{2199}
\pdfglyphtounicode{d7}{2193}
\pdfglyphtounicode{d8}{2193}
\pdfglyphtounicode{d9}{2193}
\pdfglyphtounicode{d10}{2193}
\pdfglyphtounicode{d11}{2193}
\pdfglyphtounicode{d12}{2193}
\pdfglyphtounicode{d13}{2193}
\pdfglyphtounicode{d14}{2193}
\pdfglyphtounicode{d15}{2193}
\pdfglyphtounicode{d16}{2193}
\pdfglyphtounicode{d17}{2193}
\pdfglyphtounicode{d18}{2193}
\pdfglyphtounicode{d19}{2193}
\pdfglyphtounicode{d20}{2193}
\pdfglyphtounicode{d21}{2193}
\pdfglyphtounicode{d22}{2193}
\pdfglyphtounicode{d23}{2193}
\pdfglyphtounicode{d24}{2198}
\pdfglyphtounicode{d25}{2198}
\pdfglyphtounicode{d26}{2198}
\pdfglyphtounicode{d27}{2198}
\pdfglyphtounicode{d28}{2198}
\pdfglyphtounicode{d29}{2198}
\pdfglyphtounicode{d30}{2198}
\pdfglyphtounicode{d31}{2198}
\pdfglyphtounicode{d32}{2198}
\pdfglyphtounicode{d33}{2198}
\pdfglyphtounicode{d34}{2198}
\pdfglyphtounicode{d35}{2198}
\pdfglyphtounicode{d36}{2198}
\pdfglyphtounicode{d37}{2198}
\pdfglyphtounicode{d38}{2198}
\pdfglyphtounicode{d39}{2192}
\pdfglyphtounicode{d40}{2192}
\pdfglyphtounicode{d41}{2192}
\pdfglyphtounicode{d42}{2192}
\pdfglyphtounicode{d43}{2192}
\pdfglyphtounicode{d44}{2192}
\pdfglyphtounicode{d45}{2192}
\pdfglyphtounicode{d46}{2192}
\pdfglyphtounicode{d47}{2192}
\pdfglyphtounicode{d48}{2192}
\pdfglyphtounicode{d49}{2192}
\pdfglyphtounicode{d50}{2192}
\pdfglyphtounicode{d51}{2192}
\pdfglyphtounicode{d52}{2192}
\pdfglyphtounicode{d53}{2192}
\pdfglyphtounicode{d54}{2192}
\pdfglyphtounicode{d55}{2192}
\pdfglyphtounicode{d56}{2197}
\pdfglyphtounicode{d57}{2197}
\pdfglyphtounicode{d58}{2197}
\pdfglyphtounicode{d59}{2197}
\pdfglyphtounicode{d60}{2197}
\pdfglyphtounicode{d61}{2197}
\pdfglyphtounicode{d62}{2197}
\pdfglyphtounicode{d63}{2197}
\pdfglyphtounicode{d64}{2197}
\pdfglyphtounicode{d65}{2197}
\pdfglyphtounicode{d66}{2197}
\pdfglyphtounicode{d67}{2197}
\pdfglyphtounicode{d68}{2197}
\pdfglyphtounicode{d69}{2197}
\pdfglyphtounicode{d70}{2197}
\pdfglyphtounicode{d71}{2191}
\pdfglyphtounicode{d72}{2191}
\pdfglyphtounicode{d73}{2191}
\pdfglyphtounicode{d74}{2191}
\pdfglyphtounicode{d75}{2191}
\pdfglyphtounicode{d76}{2191}
\pdfglyphtounicode{d77}{2191}
\pdfglyphtounicode{d78}{2191}
\pdfglyphtounicode{d79}{2191}
\pdfglyphtounicode{d80}{2191}
\pdfglyphtounicode{d81}{2191}
\pdfglyphtounicode{d82}{2191}
\pdfglyphtounicode{d83}{2191}
\pdfglyphtounicode{d84}{2191}
\pdfglyphtounicode{d85}{2191}
\pdfglyphtounicode{d86}{2191}
\pdfglyphtounicode{d87}{2191}
\pdfglyphtounicode{d88}{2196}
\pdfglyphtounicode{d89}{2196}
\pdfglyphtounicode{d90}{2196}
\pdfglyphtounicode{d91}{2196}
\pdfglyphtounicode{d92}{2196}
\pdfglyphtounicode{d93}{2196}
\pdfglyphtounicode{d94}{2196}
\pdfglyphtounicode{d95}{2196}
\pdfglyphtounicode{d96}{2196}
\pdfglyphtounicode{d97}{2196}
\pdfglyphtounicode{d98}{2196}
\pdfglyphtounicode{d99}{2196}
\pdfglyphtounicode{d100}{2196}
\pdfglyphtounicode{d101}{2196}
\pdfglyphtounicode{d102}{2196}
\pdfglyphtounicode{d103}{2190}
\pdfglyphtounicode{d104}{2190}
\pdfglyphtounicode{d105}{2190}
\pdfglyphtounicode{d106}{2190}
\pdfglyphtounicode{d107}{2190}
\pdfglyphtounicode{d108}{2190}
\pdfglyphtounicode{d109}{2190}
\pdfglyphtounicode{d110}{2190}
\pdfglyphtounicode{d111}{2190}
\pdfglyphtounicode{d112}{2190}
\pdfglyphtounicode{d113}{2190}
\pdfglyphtounicode{d114}{2190}
\pdfglyphtounicode{d115}{2190}
\pdfglyphtounicode{d116}{2190}
\pdfglyphtounicode{d117}{2190}
\pdfglyphtounicode{d118}{2190}
\pdfglyphtounicode{d119}{2190}
\pdfglyphtounicode{d120}{2199}
\pdfglyphtounicode{d121}{2199}
\pdfglyphtounicode{d122}{2199}
\pdfglyphtounicode{d123}{2199}
\pdfglyphtounicode{d124}{2199}
\pdfglyphtounicode{d125}{2199}
\pdfglyphtounicode{d126}{2199}
\pdfglyphtounicode{d127}{2199}
\endinput

% Reference:
%
% http://codepoints.net/basic_latin
% 0028 0029 002F 005B 005C 005D 007B 007D
%
% http://codepoints.net/spacing_modifier_letters
% 02C2 02C3 02C6 02DC
%
% http://codepoints.net/general_punctuation
% 2040 2053
%
% http://codepoints.net/letterlike_symbols
% 2127
%
% http://codepoints.net/arrows
% 2190 2191 2192 2193 2196 2197 2198 2199 219D 21A6 21A9 21AA 21D1 21D3
%
% http://codepoints.net/mathematical_operators
% 220F 2210 2211 221A 222B 222E 228F 2290 22B4 22B5 22C0 22C1 22C2 22C3
% 22C8
%
% http://codepoints.net/miscellaneous_technical
% 2303 2304 2308 2309 230A 230B 239B 239C 239D 239E 239F 23A0 23A1 23A2
% 23A3 23A4 23A5 23A6 23A7 23A8 23A9 23AA 23AB 23AC 23AD 23D0
%
% http://codepoints.net/geometric_shapes
% 25A1 25B7 25C1 25C7
%
% http://codepoints.net/miscellaneous_mathematical_symbols-a
% 27E8 27E9
%
% http://codepoints.net/supplemental_mathematical_operators
% 2A00 2A01 2A02 2A04 2A06
%
% Private Use Area:
% EB61 ED12 ED17 ED18 ED19 ED1A ED6A ED6B ED79

%
%
% End of file 'glyphtounicode-cmr.tex
%

